Counterbalancing Teacher: Regularizing Batch Normalized Models for Robustness

Batch normalization (BN) is a ubiquitous technique for training deep neural networks that accelerates their convergence to reach higher accuracy. However, we demonstrate that BN comes with a fundamental drawback: it incentivizes the model to rely on low-variance features that are highly specific to the training (in-domain) data, hurting generalization performance on out-of-domain examples. In this work, we investigate this phenomenon by first showing that removing BN layers across a wide range of architectures leads to lower out-of-domain and corruption errors at the cost of higher in-domain errors. We then propose Counterbalancing Teacher (CT), a method which leverages a frozen copy of the same model without BN as a teacher to enforce the student network's learning of robust representations by substantially adapting its weights through a consistency loss function. This regularization signal helps CT perform well in unforeseen data shifts, even without information from the target domain as in prior works. We theoretically show in an overparameterized linear regression setting why normalization leads to a model's reliance on such in-domain features, and empirically demonstrate the efficacy of CT by outperforming several baselines on robustness benchmarks such as CIFAR-10-C, CIFAR-100-C, and VLCS.

==> sections/broad.tex <==
\section{Broader impact}
\label{broder}
Despite the unprecedented success of deep learning models in a variety of machine learning (ML) applications, they have been found to be surprisingly brittle under practical, real-world scenarios that involve domain shift~\cite{galloway2019batch, khani2021removing, schneider2020improving, benz2021revisiting, hendrycks2019augmix, vasiljevic2016examining, hendrycks2019benchmarking, madry2017towards, rusak2020simple, dodge2017quality, goldblum2020adversarially, hendrycks2019using}. In this work, we proposed a representation learning framework to help mitigate such failures by encouraging the neural network to learn features that generalize in common OOD settings, such as data corruptions. However, the risks and consequences that come with deploying ML systems in high-stakes applications such as automated manufacturing, autonomous vehicles, and medical diagnostics are still high. Though our approach demonstrates an improvement in a selection of OOD settings, there is still much work to be done in this space in order to make sure that ML systems are safe and reliable in all test scenarios.



==> sections/checklist.tex <==
% \section*{Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

% \begin{enumerate}

% \item For all authors...
% \begin{enumerate}
%   \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
%     \answerYes{}
%   \item Did you describe the limitations of your work?
%     \answerYes{} See end of the method section. 
%   \item Did you discuss any potential negative societal impacts of your work?
%     \answerYes{} See the Broader Impact Section
%   \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
%     \answerYes{}
% \end{enumerate}

% \item If you are including theoretical results...
% \begin{enumerate}
%   \item Did you state the full set of assumptions of all theoretical results?
%     \answerYes{}
% 	\item Did you include complete proofs of all theoretical results?
%     \answerYes{}
% \end{enumerate}

% \item If you ran experiments...
% \begin{enumerate}
%   \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
%     \answerYes{} We will provide the code in supplementary material. We provided instructions on how to run our experiments e.g. datasets, hyper-parameters. 
%   \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
%     \answerYes{} Hyper-parameters are reported in the Appendix.
% 	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
%     \answerNo{} We ran several experiments multiple times (e.g. the MNIST and OOD experiments), but to be consistent with how the previous methods reported their results we reported mean values.
% 	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
%     \answerNo{}
% \end{enumerate}

% \item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
% \begin{enumerate}
%   \item If your work uses existing assets, did you cite the creators?
%     \answerYes{}
%   \item Did you mention the license of the assets?
%     \answerNA{}
%   \item Did you include any new assets either in the supplemental material or as a URL?
%     \answerNA{}
%   \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
%     \answerNA{}
%   \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
%     \answerNA{}
% \end{enumerate}

% \item If you used crowdsourcing or conducted research with human subjects...
% \begin{enumerate}
%   \item Did you include the full text of instructions given to participants and screenshots, if applicable?
%     \answerNA{}
%   \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
%     \answerNA{}
%   \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
%     \answerNA{}
% \end{enumerate}

% \end{enumerate}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/implementation_details.tex <==
\section{Implementation details}



We implement our CT variants using Tensorflow~\cite{abadi2016tensorflow}. We train the self-supervised methods with batch size 256 for 1000 epochs while maintaining the original hyper-parameters. We fine-tune all self-supervised methods for 350 epochs with Adam~\cite{kingma2014adam} and with starting learning rate of 0.001 with a cosine decay, and $l_2$ coefficient set to 0.0005 to avoid overfitting. 

1- Model architecture for MNIST experiment\\
2- Hyper-params of CT for different experiments



==> sections/prelims.tex <==
% \section{Preliminaries}
% \label{prelims}


\section{Problem statement and analysis}
\looseness=-1
We assume a supervised classification setting: given an input variable $x \in \mathcal{X} 	\subseteq \mathbb{R}^d$, and a set of corresponding labels $y \in \mathcal{Y} = \{1, ..., k\}$, we aim to learn a classifier $f_{\zeta}: \mathcal{X} \longrightarrow \mathcal{Y}$ by minimizing the empirical risk: \kristy{! check notation with theory}


\begin{equation}
\begin{split}
  \zeta &= \operatorname*{argmin}_\zeta \mathbb{E}_{x, y \sim p_{d}(x, y)}[\ell(x, y; \zeta)] \\
  & \approx \operatorname*{argmin}_\zeta \sum_{i=1}^{n} \ell(f_{\zeta}(x_i), y_i) 
\end{split}
\label{eqn:nn_real_model}
\end{equation} 
Here $p_d(x, y)$ is the underlying joint distribution from where the dataset $ \mathcal{D} = \{(x_i, y_i)\}_{i=1}^n$ is sampled. In the following sections, we first discuss the effect of (batch) normalization on the solutions found in underspecified regimes, then elaborate on our approach to optimize the aforementioned empirical risk. In this context, we refer to a problem as underspecified or overparameterized when degrees of freedom of a model is larger than the number of training examples.

